Flexible Techniques for Differentiable Rendering with 3D Gaussians

Fast, reliable shape reconstruction is an essential ingredient in many computer vision applications. Neural Radiance Fields demonstrated that photorealistic novel view synthesis is within reach, but was gated by performance requirements for fast reconstruction of real scenes and objects. Several recent approaches have built on alternative shape representations, in particular, 3D Gaussians. We develop extensions to these renderers, such as integrating differentiable optical flow, exporting watertight meshes and rendering per-ray normals. Additionally, we show how two of the recent methods are interoperable with each other. These reconstructions are quick, robust, and easily performed on GPU or CPU. For code and visual examples, see https://leonidk.github.io/fmb-plus

==> page_fig.tex <==
%\begin{table*}[tbhp]
%\centering
\begin{table}[thbp]%{0.49\linewidth}
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
 & \multicolumn{2}{l}{\textbf{Ficus}} & \multicolumn{2}{l}{\textbf{CO3D Teddy}} \\ 
  & \multicolumn{2}{l}{ (25,778 Gaussians)} & \multicolumn{2}{l}{(40 Gaussians)} \\ \midrule

 & CPU & GPU & CPU & GPU \\
 Blending \\(\Cref{sec:weightb}) & 4.43 ms & 38.5 ns & 1.63 $\mu$s & 10.7 ns \\ 
 Compositing\\ (\Cref{sec:alphac}) & 25.2 ms & 43.9 ns & 8.50 $\mu$s &  13.6 ns\\ \bottomrule
\end{tabular}
\caption{\textbf{Runtimes for rendering forward passes} for a single ray with a i5-7267U CPU and a GTX 1080 GPU. The smaller differences in GPU runtime suggest the approach is more memory limited and not compute bound in our current implementation.}
\label{tab:runtimes_fwd}
\end{table}
%\hfill

%\caption{\textbf{Runtime experiments} analyzing the approaches described in \Cref{sec:rayshape}.}
%\label{tab:runtime_both}
%\end{table*}

